UniPCGC: Towards Practical Point Cloud Geometry Compression via an Efficient Unified Approach

Learning-based point cloud compression methods have made significant progress in terms of performance. However, these methods still encounter challenges including high complexity, limited compression modes, and a lack of support for variable rate, which restrict the practical application of these methods. In order to promote the development of practical point cloud compression, we propose an efficient unified point cloud geometry compression framework, dubbed as UniPCGC. It is a lightweight framework that supports lossy compression, lossless compression, variable rate and variable complexity. First, we introduce the Uneven 8-Stage Lossless Coder (UELC) in the lossless mode, which allocates more computational complexity to groups with higher coding difficulty, and merges groups with lower coding difficulty. Second, Variable Rate and Complexity Module (VRCM) is achieved in the lossy mode through joint adoption of a rate modulation module and dynamic sparse convolution. Finally, through the dynamic combination of UELC and VRCM, we achieve lossy compression, lossless compression, variable rate and complexity within a unified framework. Compared to the previous state-of-the-art method, our method achieves a compression ratio (CR) gain of 8.1\% on lossless compression, and a Bjontegaard Delta Rate (BD-Rate) gain of 14.02\% on lossy compression, while also supporting variable rate and variable complexity.

==> table/lossless1.tex <==
\begin{table*}[]
\caption{{Quantitative performance gains to the G-PCC and SparsePCGC. Compression ratio (CR) gain is measured by bits per point (bpp).}}
\label{table:lossless1}
\centering
\begin{tabular}{|ccccccccc|}
\hline
\multicolumn{1}{|c|}{\multirow{3}{*}{\textbf{Point Clouds}}} & \multicolumn{8}{c|}{\textbf{lossless}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             \\ \cline{2-9} 
\multicolumn{1}{|c|}{}                                       & \multicolumn{2}{c|}{\textbf{G-PCC}}                                                                                          & \multicolumn{2}{c|}{\textbf{SparsePCGC}}                                                                                     & \multicolumn{2}{c|}{\textbf{Ours}}                                                                                             & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}CR-gain\\ (G-PCC)\end{tabular}}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}CR-gain\\ (SparsePCGC)\end{tabular}}} \\ \cline{2-7}
\multicolumn{1}{|c|}{}                                       & \multicolumn{1}{c|}{\textbf{bpp}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Time (s)\\ Enc/Dec\end{tabular}}} & \multicolumn{1}{c|}{\textbf{bpp}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Time (s)\\ Enc/Dec\end{tabular}}} & \multicolumn{1}{c|}{\textbf{bpp}}   & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Time (s)\\ Enc/Dec\end{tabular}}} & \multicolumn{1}{c|}{}                                                                                    &                                                                                          \\ \hline
% \multicolumn{9}{|c|}{\textbf{Dense Object}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       \\ \hline
\multicolumn{1}{|c|}{basketball\_player\_vox11}              & \multicolumn{1}{c|}{0.646}        & \multicolumn{1}{c|}{8.64/5.18}                                                           & \multicolumn{1}{c|}{0.501}        & \multicolumn{1}{c|}{1.51/1.47}                                                           & \multicolumn{1}{c|}{0.470}          & \multicolumn{1}{c|}{1.32/1.30}                                                           & \multicolumn{1}{c|}{-27.2\%}                                                                             & -6.2\%                                                                                   \\ 
\multicolumn{1}{|c|}{dancer\_vox11}                          & \multicolumn{1}{c|}{0.629}        & \multicolumn{1}{c|}{7.40/4.57}                                                           & \multicolumn{1}{c|}{0.502}        & \multicolumn{1}{c|}{1.38/1.34}                                                           & \multicolumn{1}{c|}{0.466}          & \multicolumn{1}{c|}{1.14/1.13}                                                           & \multicolumn{1}{c|}{-25.9\%}                                                                             & -7.2\%                                                                                   \\ 
\multicolumn{1}{|c|}{longdress\_vox10}                       & \multicolumn{1}{c|}{0.740}        & \multicolumn{1}{c|}{2.25/1.52}                                                           & \multicolumn{1}{c|}{0.639}        & \multicolumn{1}{c|}{0.56/0.50}                                                           & \multicolumn{1}{c|}{0.610}          & \multicolumn{1}{c|}{0.66/0.48}                                                           & \multicolumn{1}{c|}{-17.6\%}                                                                             & -4.5\%                                                                                   \\ 
\multicolumn{1}{|c|}{loot\_vox10}                      & \multicolumn{1}{c|}{0.702}        & \multicolumn{1}{c|}{2.09/1.42}                                                           & \multicolumn{1}{c|}{0.606}        & \multicolumn{1}{c|}{0.54/0.49}                                                           & \multicolumn{1}{c|}{0.581}          & \multicolumn{1}{c|}{0.50/0.45}                                                           & \multicolumn{1}{c|}{-17.2\%}                                                                             & -4.1\%                                                                                   \\ 
\multicolumn{1}{|c|}{queen\_0200}                            & \multicolumn{1}{c|}{0.604}        & \multicolumn{1}{c|}{2.60/1.71}                                                           & \multicolumn{1}{c|}{0.556}        & \multicolumn{1}{c|}{0.65/0.59}                                                           & \multicolumn{1}{c|}{0.496}          & \multicolumn{1}{c|}{0.56/0.51}                                                           & \multicolumn{1}{c|}{-17.8\%}                                                                             & -10.8\%                                                                                   \\ 
\multicolumn{1}{|c|}{redandblack\_vox10}               & \multicolumn{1}{c|}{0.823}        & \multicolumn{1}{c|}{1.99/1.36}                                                           & \multicolumn{1}{c|}{0.708}        & \multicolumn{1}{c|}{0.62/0.50}                                                           & \multicolumn{1}{c|}{0.686}          & \multicolumn{1}{c|}{0.61/0.48}                                                           & \multicolumn{1}{c|}{-25.9\%}                                                                             & -3.1\%                                                                                   \\ 
\multicolumn{1}{|c|}{soldier\_vox10}                         & \multicolumn{1}{c|}{0.737}        & \multicolumn{1}{c|}{2.86/1.93}                                                           & \multicolumn{1}{c|}{0.643}        & \multicolumn{1}{c|}{0.66/0.62}                                                           & \multicolumn{1}{c|}{0.619}          & \multicolumn{1}{c|}{0.60/0.57}                                                           & \multicolumn{1}{c|}{-19.1\%}                                                                             & -4.2\%                                                                                   \\ \hline
\multicolumn{1}{|c|}{\textbf{Average}}                       & \multicolumn{1}{c|}{0.697}        & \multicolumn{1}{c|}{3.97/2.53}                                                           & \multicolumn{1}{c|}{0.594}        & \multicolumn{1}{c|}{0.84/0.79}                                                           & \multicolumn{1}{c|}{\textbf{0.561}} & \multicolumn{1}{c|}{\textbf{0.77/0.70}}                                                  & \multicolumn{1}{c|}{\textbf{-19.6\%}}                                                                    & \textbf{-5.6\%}                                                                          \\ \hline
\end{tabular}
\end{table*}

==> table/lossless_8i_device.tex <==
\begin{table*}[]
\caption{Performance of \textbf{lossless methods} on the 8iVFB testset under the same training conditions. The performance numbers of the compared methods are directly cited from \cite{sparsepcgc,ecm,gao2022openpointcloud}. Due to the lack of the same GPU device as \cite{sparsepcgc,ecm} for runtime testing, UniPCGC and SparsePCGC are tested using RTX 4080 GPU and intel i5-13600KF CPU for a fair runtime comparison (Mark with *).}
\label{table:lossless_8i_device}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\textbf{Point clouds} & \textbf{Ours}  & \textbf{GPCC} & \textbf{SparsePCGC} & \textbf{VoxelDNN} & \textbf{MsVoxel} & \textbf{OctAttention} & \textbf{ECM} \\ \hline
Red\&black            & 0.59           & 0.82         & 0.64                & 0.67         & 0.87            & 0.73                  & 0.66              \\
Loot                  & 0.49           & 0.69         & 0.53                & 0.58         & 0.73            & 0.62                  & 0.55              \\
Thaidancer            & 0.51           & 0.70         & 0.56                & 0.68         & 0.85            & 0.65                  & 0.58              \\
Boxer                 & 0.45           & 0.65         & 0.49                & 0.55          & 0.70             & 0.59                  & 0.51              \\ \hline

\textbf{Average Bpp}  & \textbf{0.51}  & 0.72        & 0.56               & 0.62       & 0.79          & 0.65                & 0.58             \\ \hline
\textbf{Ours CR Gain} & \textbf{0.0\%} & -29.2\%       & -8.1\%              & -17.4\%       & -35.2\%         & -21.2\%               & -11.3\%           \\ \hline
\textbf{Enc time(s)}  & *0.56   & *1.99          & *0.71/2.09                 & 885           & 54              & 1.06                  & 1.92              \\ \hline
\textbf{Dec time(s)}  & *0.57  & *1.49          & *0.88/1.91                 & 640           & 58              & 1229                  & 19.5              \\ \hline
\textbf{Test Device}  & RTX4080  & RTX4080          & RTX4080/2080                 & RTX2080           & RTX2080              & RTX2080                  & RTX3090              \\ \hline
\textbf{Model Size(M)}  & 2.3  & /          & 5.0                 & 3.4           & 13.0              & 18.1                   & /              \\ \hline
\end{tabular}
\end{table*}

==> table/lossy_abla.tex <==
\begin{table}[]
\caption{The ablation experiments of VRCM on the selected dense point clouds. 
UELC represents Uneven 8-Stage Lossless Coder, VR represents Variable Rate Module, VC represents Variable Complexity Module, and \checkmark denotes the usage of that method. D1-Gain represents the BD(D1)-rate gain over the baseline, D2-Gain represents the BD(D2)-rate gain over the baseline. }
\label{table:ablation_lossy}
\centering
\begin{tabular}{|c|ccc|c|c|}
\hline
\textbf{Method}                & \textbf{UELC} & \textbf{VR} & \textbf{VC} & \textbf{D1-Gain }  & \textbf{D2-Gain}  \\ \hline
Base           &   &              &             & 0.0\%   & 0.0\%        \\
UELC                 &          \checkmark     &   &             & -2.03\%     & -2.09\%     \\
VRM                &  \checkmark           &         \checkmark     &   & -8.20\%  & -7.07\%         \\
\textbf{VRCM} &     \checkmark        & \checkmark   & \checkmark  & \textbf{-14.02\%} & \textbf{-12.20\%}  \\ \hline
\end{tabular}
\end{table}

==> table/lossy_all.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\caption{{BD-Rate gains measured using both D1 and D2 for the UniPCGC against the PCGCv2, ADL-PCC, GeoCNNv2, SparsePCGC, G-PCC and G-PCC (Trisoup) for lossy compression}.}
\label{table:lossy_all}
\centering
\begin{tabular}{|c|cc|cc|cc|cc|cc|cc|}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Point\\ Cloud\end{tabular}}} & \multicolumn{2}{c|}{\textbf{PCGCv2}} & \multicolumn{2}{c|}{\textbf{ADL-PCC}} & \multicolumn{2}{c|}{\textbf{GeoCNNv2}} & \multicolumn{2}{c|}{\textbf{SparsePCGC}} & \multicolumn{2}{c|}{\textbf{G-PCC}} & \multicolumn{2}{c|}{\textbf{G-PCC (T)}} \\ \cline{2-13} 
                                                                                & \textbf{D1}       & \textbf{D2}      & \textbf{D1}       & \textbf{D2}       & \textbf{D1}        & \textbf{D2}       & \textbf{D1}         & \textbf{D2}        & \textbf{D1}      & \textbf{D2}      & \textbf{D1}        & \textbf{D2}        \\ \hline
\textbf{long}                                                              & -49.9\%           & -39.7\%          & -77.5\%           & -75.9\%           & -75.7\%            & -71.5\%           & -13.1\%             & -13.6\%            & -94.9\%          & -90.4\%          & -87.1\%            & -80.4\%            \\
\textbf{loot}                                                                   & -47.7\%           & -31.9\%          & -70.2\%           & -69.1\%           & -73.3\%            & -67.1\%           & -7.2\%              & -6.2\%             & -94.1\%          & -88.8\%          & -88\%              & -79.1\%            \\
\textbf{red}                                                             & -47.3\%           & -36.9\%          & -73.5\%           & -71.7\%           & -73.9\%            & -69.3\%           & -13.4\%             & -11.3\%            & -94.5\%          & -89.6\%          & -87.4\%            & -79.9\%            \\
\textbf{soldier}                                                                & -50.1\%           & -40.7\%          & -78.2\%           & -76.6\%           & -76.7\%            & -72.2\%           & -15.9\%             & -13.4\%            & -95.4\%          & -91.3\%          & -90\%              & -84.1\%            \\
\textbf{queen}                                                                  & -38.9\%           & -33.7\%          & -78.5\%           & -78.1\%           & -73.9\%            & -68.7\%           & -9.2\%              & -10.0\%            & -95.4\%          & -90.8\%          & -90.1\%            & -79.9\%            \\
\textbf{player}                                                                 & -51.1\%           & -45.0\%          & -82.8\%           & -81.6\%           & -80.8\%            & -77.4\%           & -11.9\%             & -11.7\%            & -97.3\%          & -95.1\%          & -95.4\%            & -89.5\%            \\
\textbf{dancer}                                                                 & -52.4\%           & -44.7\%          & -81.6\%           & -78.7\%           & -79.4\%            & -73.9\%           & -13.1\%             & -12.0\%            & -97\%            & -94.2\%          & -94.2\%            & -87.2\%            \\ \hline
\textbf{Average}                                                                & \textbf{-48.2\%}  & \textbf{-38.9\%} & \textbf{-77.5\%}  & \textbf{-76.0\%}  & \textbf{-76.2\%}   & \textbf{-71.4\%}  & \textbf{-12.0\%}    & \textbf{-11.2\%}   & \textbf{-95.5\%} & \textbf{-91.5\%} & \textbf{-90.3\%}   & \textbf{-82.9\%}   \\ \hline
\end{tabular}
\end{table*}

==> table/lossy_gpcc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{{BD-Rate gains measured using both D1 and D2 for the UniPCGC against the G-PCC v23 for lossy coded dense point clouds}}
\label{table:lossy_gpcc}
\centering
\begin{tabular}{ccc}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Dense\\ Point Clouds\end{tabular}}}}           & \multicolumn{2}{c|}{\textbf{G-PCC}}                           \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                                                                       & \textbf{D1}          & \multicolumn{1}{c|}{\textbf{D2}} \\   \hline
\multicolumn{1}{|c|}{longdress\_vox10\_1300}                                                                        & -92.41\%             & \multicolumn{1}{c|}{-87.08\%}          \\
\multicolumn{1}{|c|}{loot\_vox10\_1200}                                                                             & -92.97\%             & \multicolumn{1}{c|}{-87.79\%}          \\
\multicolumn{1}{|c|}{red\&black\_vox10\_1550}                                                                     & -91.33\%             & \multicolumn{1}{c|}{-85.13\%}          \\
\multicolumn{1}{|c|}{soldier\_vox10\_0690}                                                                        & -91.65\%             & \multicolumn{1}{c|}{-86.14\%}          \\
\multicolumn{1}{|c|}{queen\_0200}                                                                                   & -93.51\%             & \multicolumn{1}{c|}{-88.79\%}          \\
\multicolumn{1}{|c|}{player\_vox11\_200}                                                                             & -95.77\%             & \multicolumn{1}{c|}{-92.99\%}          \\
\multicolumn{1}{|c|}{dancer\_vox11\_0001}                                                                        & -95.43\%             & \multicolumn{1}{c|}{-91.40\%}          \\ \hline
\multicolumn{1}{|c|}{\textbf{Average}}                                                                      & \textbf{-93.30\%}    & \multicolumn{1}{c|}{\textbf{-88.47\%}} \\ \hline
\multicolumn{1}{l}{}                                                                                                      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}                   \\
\multicolumn{1}{l}{}                                                                                                        & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}                  
\end{tabular}
\end{table}


==> table/lossy_runtime.tex <==
\begin{table*}[]
\caption{Performance comparison of \textbf{lossy compression}. Decoding time, model size, and RD-Rate gain are all displayed. UniPCGC, SparsePCGC \cite{sparsepcgc}, PCGCv2 \cite{pcgcv2}, ADL-PCC \cite{adl_pcc}, GeoCNNv2 \cite{geocnnv2} and G-PCC are all compared.}
\label{table:lossy_runtime}
\centering
\begin{tabular}{ccccccc}
\toprule
                               & \textbf{Ours} & \textbf{PCGCv2} & \textbf{SparsePCGC} & \textbf{ADL-PCC} & \textbf{GeoCNNv2} & \textbf{G-PCC} \\ \midrule
\textbf{Dec time(s)}           & 0.74          & 0.53            & 0.73                & 14.63            & 58                    & 1.16           \\
\textbf{Test Device}           & RTX4080       & RTX4080         & RTX4080             & RTX2080 Ti       & RTX2080 Ti            & RTX4080        \\
\textbf{Model Size(M)}         & 7.6           & 3.2             & 9.5                 & 32.8             & 18.8                  & /              \\
\textbf{Ours BD(D1)-Rate Gain} & /             & -49.75\%         & -14.02\%             & -77.93\%          & -75.94\%               & -93.30\%        \\
\textbf{Ours BD(D2)-Rate Gain} & /             & -42.00\%         & -12.20\%             & -76.36\%          & -70.43\%               & -88.47\%        \\ \bottomrule
\end{tabular}
\end{table*}
